Augmented CycleGAN: Learning Many-to-Many Mappings from Unpaired Data

Learning inter-domain mappings from unpaired data can improve performance in structured prediction tasks, such as image segmentation, by reducing the need for paired data. CycleGAN was recently proposed for this problem, but critically assumes the underlying inter-domain mapping is approximately deterministic and one-to-one. This assumption renders the model ineffective for tasks requiring flexible, many-to-many mappings. We propose a new model, called Augmented CycleGAN, which learns many-to-many mappings between domains. We examine Augmented CycleGAN qualitatively and quantitatively on several image datasets.

==> 5-experiments-old.tex <==

\section{Experiments} \label{sec:experiments}



\subsection{Edges-to-Photos} \label{sec:e2s_experiments}
We first study a one-to-many image translation task between edges (domain $\A$) and photos of shoes (domain $\B$). 
%The relationship between (domain $\A$) and shoes (domain $\B$) is one-to-many, as there many possible images of shoes that can be associated with a given edge image.
Training data is composed of almost 50K shoe images with corresponding edges~\citep{yu2014fine,zhu2016generative,isola2017image}, but as in previous approaches (e.g. \citep{kim2017learning}), we assume no pairing information while training unsupervised models. Stochastic mappings in our Augmented CycleGAN (AugCGAN) model are based on ResNet conditional image generators of~\citep{zhu2017unpaired}, where we inject noise with CIN to all intermediate layers.~\footnote{Architecture and training details of this experiment are provided in Sec.\todo{name section.}}
%of $\Fz$, and use a deterministic mapping from shoes to edges, i.e. $\Gz=\G$, since the relationship is one-to-many. 
As baselines, we train: CycleGAN, Stochastic CycleGAN (StochCGAN) and Triangle-GAN ($\Delta$-GAN) of~\citep{gan2017triangle} which share the same architectures and training procedure for fair comparison.~\footnote{$\Delta$-GAN architecture differs only in the two discriminators, which match conditionals/joints instead of marginals.}

\begin{table*}[t]
\centering
\begin{minipage}[t]{.45\textwidth}
%  \begin{minipage}[b]{.22\textwidth}
  \subfloat[AugCGAN]
  {\includegraphics[width=0.45\textwidth]{FIG/edges2shoes/aug_cgan_short/multi_1.png}}
  \hfill
%  \end{minipage}
%\begin{minipage}[b]{.22\textwidth}
  \subfloat[StochCGAN]
  {\includegraphics[width=0.45\textwidth]{FIG/edges2shoes/stoch_cgan_short/multi_2.png}}
%  \end{minipage}
\captionof{figure}{We start from an edge sampled from the data distribution (leftmost column) and generate multiple shoes by sampling five different $z_b \sim \pz(z_b)$. Both models generate diverse shoes when edges are sampled from the data distribution.}
\label{fig:e2s_multi}
\end{minipage}
\hfill
\begin{minipage}[t]{.49\textwidth}
  \subfloat[AugCGAN]
  {\includegraphics[width=0.45\textwidth]{FIG/edges2shoes/aug_cgan_short/cycle_short.png}}
  \hfill
  \subfloat[StochCGAN]
  {\includegraphics[width=0.45\textwidth]{FIG/edges2shoes/stoch_cgan_short/cycle_short.png}}
\captionof{figure}{Cycles from both models starting from a real edge and a real shoe (left and right respectively in each subfigure). The ability for StochCGAN to reconstruct shoes is surprising and is due to the ``steganography'' effect (see text).}
\label{fig:e2s_cycle}
\end{minipage}
\end{table*}


\paragraph{Qualitative Results} 
First we qualitatively compare the mappings learned by our model AugCGAN and StochCGAN. Fig.~\ref{fig:e2s_cycle} shows generated images from of shoes given an edge $a \sim \pdata(a)$ (row) and $z_b \sim p(z_b)$ (column) from both model, and Fig.~\ref{fig:e2s_multi} shows cycles starting from edges and shoes. Note that here the edges are sampled from the data distribution and not produced by the learnt stochastic mapping $\G$.
In this case, both models can
\begin{inlinelist}
\item generate diverse set of shoes with color variations mostly defined by $z_b$, and
\item perform reconstructions of both edges and shoes.
\end{inlinelist}
While we expect our model to achieve these results, the fact that StochCGAN can reconstruct shoes perfectly without an inference model may seem at first surprising. This effect can be explained by the ``steganography" behavior of CycleGAN~\citep{chu2017cyclegan}: the model hides in the generated edge $\tilde{a}$ imperceptible information about a given shoe $b$ (for example, its color), in order to satisfy cycle-consistency without being penalized by the discriminator on $\A$.
Based on these considerations, we perform an additional experiment: a good model of the true conditional mappings $p(b|a)$, $p(a|b)$ between domains should be able to reproduce the hidden joint distribution and consequently, the observed marginals, by alternatively sampling from the conditionals. Therefore, we examine the behavior of the models when edges are generated from the model itself (instead of sampled from the empirical data distribution). In Fig.~\ref{fig:e2s_cycle_B_multi}, we plot
multiple generated shoes given an edge generated by the model $\tilde{a}$ and 5 different $z_b$ sampled from \text{prior} $p(z_b)$. In StochCGAN, the mapping $\Gz(\tilde{a}, z_b)$ collapses to a deterministic function generating a single shoe for every $z_b$. In AugCGAN, on the other hand, the mapping seem to closely capture the diversity in the conditional distribution of shoes given edges.
% does not collapse and generate a diverse set of reconstructed shoes sharing the same shape of the original shoe but with colors captured by $z_b$.
Furthermore, in Fig.~\ref{fig:e2s_multi_cycle}, we run a markov chain by generating from the learnt mappings multiple times, starting from a real shoe. Again AugCGAN produces diverse reconstructions while StochCGAN seems to collapse to a single mode of the conditional distribution.
%Fig.~\ref{fig:e2s_multi_cycle} provides another comparison between AugCGAN and StochCGAN multiple cycles through each model, where start from a real shoe and reconstruct it with $z_b \sim p(z_b)$ in every cycle step.

\paragraph{Quantitative Results}
We  investigate ``steganography'' behavior in both AugCGAN and StochCGAN using a similar approach to~\citep{chu2017cyclegan}, where we corrupt generated edges with noise sampled from $\mathcal{N}(0,\epsilon^2)$, and compute reconstruction error of original edges after corruption. Fig.~\ref{fig:noise_sensitivity} shows $L_1$ reconstruction error as we increase $\epsilon$. We can see that while our AugCGAN  model is also subject to some ``steganography'', shoe reconstructions are more robust to corruption of edges than in StochCGAN, which is a result of encoding information about shoes in the latent code, and confirms that learning mappings over augmented spaces help with easing information bottleneck imposed by the restricted edge domain.
Secondly, we evaluate conditionals learned by each model by measuring the likelihood of generating a specific edge-shoe pair from a test set. 
While in GAN-based models we cannot compute likelihoods tractably, we follow an inference-via-optimization approach similar to~\citep{metz2016unrolled,xiang2017effects} to estimate the likelihood of generating a specific shoe given and edge. Specifically, given a trained model with mapping $\Fz$ and an edge-shoe pair $(a,b)$ in the test set, we solve the optimization task $z_b^* = \argmin_{z_b} \| \Fz(a,z_b) - b \|_1$ and compute prediction error\footnote{\todo{should we call it reconstruction loss or prediction loss? I find reconstruction loss confusing a bit.}} $\| \Fz(a,z_b^*)-b\|_1$. Optimization is done with RMSProp as in~\citep{xiang2017effects}. We show the average errors over a predefined test set of 200 samples in Table~\ref{tab:shoe_recons} for: AugCGAN (unsupervised and semi-supervised with 10\% paired data), unsupervised CycleGAN and StochCGAN, and a semi-supervised $\Delta$-GAN, all sharing the same architecture. Our unsupervised AugCGAN model outperforms all baselines including semi-supervised $\Delta$-GAN, which indicates that reconstruction-based cycle-consistency is more effective in learning conditionals than the adversarial approach of $\Delta$-GAN. 
As expected, adding 10\% supervision to AugCGAN improves shoe predictions further. 
In addition, we evaluate edge predictions given real shoes from test set as well. We report mean squared error (MSE) similar to~\citep{gan2017triangle}, where we normalize over all edge pixels. The $\Delta$-GAN model with our architecture outperforms the one reported in~\citep{gan2017triangle}, but is outperformed by our unsupervised AugCGAN model. Again, adding 10\% supervision to AugCGAN reduces MSE even further.

\begin{figure}
\centering
  \begin{minipage}[b]{.22\textwidth}
  %\subfloat[AugCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/aug_cgan_short/cycle_B_multi_1.png}}
  \subfloat[AugCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/aug_cgan/cycle_B_multi_1.png}}
  \end{minipage}
\begin{minipage}[b]{.22\textwidth}
  %\subfloat[StochCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/stoch_cgan_short/cycle_B_multi_0.png}}
  \subfloat[StochCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/stoch_cgan/cycle_B_multi_0.png}}
  \end{minipage}
\caption{We start by a shoe coming from the data distribution (leftmost column) and we generate an edge (second column). Then, we generate multiple shoes by sampling five different $z_b \sim p(z_b)$. When edges are generated by the model, StochCGAN collapses to a single mode.}
\label{fig:e2s_cycle_B_multi}
\end{figure}
\begin{figure}
\centering
  \begin{minipage}[b]{.23\textwidth}
  \subfloat[AugCGAN]{\includegraphics[width=0.95\textwidth]{FIG/edges2shoes/aug_cgan/multi_cycle_1.png}}
  \end{minipage}
\begin{minipage}[b]{.23\textwidth}
  \subfloat[StochCGAN]{\includegraphics[width=0.95\textwidth]{FIG/edges2shoes/stoch_cgan/multi_cycle_0.png}}
  \end{minipage}
\caption{We perform multiple generation cycles from the model by sequential application of the learned mappings. StochCGAN cycles collapse to generating the same shoe in each step which indicates that the model doesn't capture the data distribution.}
\label{fig:e2s_multi_cycle}
\end{figure}

\begin{table*}[t!]
\begin{minipage}[b]{.35\linewidth}
\centering
\includegraphics[width=\linewidth]{FIG/edges2shoes/noise_sensitivity.pdf}
\captionof{figure}{Sensitivity to corruption.}
    \label{fig:noise_sensitivity}
\end{minipage}
\hfill
\begin{minipage}[b]{.3\linewidth}
\centering
\begin{tabular}{lcc}
    \toprule
    Model (Paired \%)    &   Avg. $L_1$\\
    \midrule
    CycleGAN  (0\%)& 0.1837 \\
    StochCGAN (0\%) & 0.0794 \\
    $\Delta$-GAN$^\dagger$ (10\%)  & 0.0748 \\
    \midrule
    AugCGAN  (0\%) & \textbf{0.0698} \\
	AugCGAN (10\%)  & \textbf{0.0562} \\
    \bottomrule
  \end{tabular}
  \caption{Shoe prediction errors. $^\dagger$Our architecture.}
  \label{tab:shoe_recons}
\end{minipage}
% \begin{minipage}[b]{.3\linewidth}
% \centering
% \begin{tabular}{lcc}
%     \toprule
%     Model (Paired Data)    &  BPP &  $L_1$\\
%     \midrule
%     CycleGAN  (0\%)& 6.77 & 0.1837 \\
%     StochCGAN (0\%) & 5.53 & 0.0794 \\
%     AugCGAN  (0\%) & 5.43 & 0.0698 \\
%     $\Delta$-GAN$^\dagger$ (10\%)   & 5.48 & 0.0748 \\
% 	AugCGAN (10\%)  & 5.13 & 0.0562 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Shoe likelihood. $^\dagger$ Our implementation.}
% \end{minipage}
\hfill
\begin{minipage}[b]{.3\linewidth}
\centering
\begin{tabular}{lc}
    \toprule
    Model (Paired \%)    & MSE\\
    \midrule
    $\Delta$-GAN$^\star$ (10\%)  & 0.0102 \\
    $\Delta$-GAN$^\dagger$ (10\%)  & 0.0096 \\
    $\Delta$-GAN$^\star$ (20\%) & 0.0092 \\
    \midrule
    AugCGAN (0\%)   & \textbf{0.0079} \\
    AugCGAN (10\%)  & \textbf{0.0052} \\
    \bottomrule
  \end{tabular}
  \caption{Edge MSE. $^\star$From \citep{gan2017triangle}. $^\dagger$Our architecture.}
   \label{tab:edge_recons}
\end{minipage} 
\end{table*}

% \begin{table*}[t]
% \begin{minipage}[b]{.4\linewidth}
% \centering
% \includegraphics[width=\linewidth]{FIG/edges2shoes/noise_sensitivity.pdf}
% \captionof{figure}{Sensitivity to corruption.}
%     \label{fig:noise_sensitivity}
% \end{minipage}
% \hfill
% \end{table*}


% \begin{figure}
% \centering
%   \begin{minipage}[b]{.2\textwidth}
%   \subfloat[AugCGAN]
%   {\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/aug_cgan_short/multi_1.png}}
%   %{\label{fig:e2s_augcgan_multi}\includegraphics[width=0.9\textwidth,trim={0 11.65cm 0 0},clip]{FIG/edges2shoes/aug_cgan/multi_1.png}}
%   \end{minipage}
% \begin{minipage}[b]{.2\textwidth}
%   \subfloat[StochCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/stoch_cgan_short/multi_2.png}}
%   \end{minipage}
% \caption{Shoe samples given edges and $z_b \sim \pz(z_b)$ shared across rows. Both models generate diverse shoes.}
% \label{fig:e2s_multi}
% \end{figure}

% \begin{figure}
% \centering
%   \begin{minipage}[b]{.22\textwidth}
%   \subfloat[AugCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/aug_cgan_short/cycle_short.png}}
%   \end{minipage}
% \begin{minipage}[b]{.22\textwidth}
%   \subfloat[StochCGAN]{\includegraphics[width=0.9\textwidth]{FIG/edges2shoes/stoch_cgan_short/cycle_short.png}}
%   \end{minipage}
% \caption{Forward and Backward Cycles. Both models can perform good reconstructions.}
% \label{fig:e2s_cycle}
% \end{figure}

\subsection{Male-to-Female} \label{sec:m2f_experiments}




\begin{figure}

  \begin{minipage}[b]{\textwidth}
  
  \subfloat[AugCGAN]{\includegraphics[width=.45\textwidth]{FIG/male2female/aug_cgan/multi_128_28.png}}
  \end{minipage}
  \caption{We start from a male face from the data distribution (leftmost column) and generate 8 different female faces by sampling $z_b \sim p(z_b)$.}
  \label{fig:m2f_128}
  \end{figure}

\begin{figure*}[th]
\centering
  \begin{minipage}[b]{\textwidth}
  \centering
  \subfloat[AugCGAN Male-to-Female]{\includegraphics[width=.24\textwidth]{FIG/male2female/aug_cgan/multi_A_B.png}}
  \hfill
%   \includegraphics[width=0.47\textwidth]{FIG/male2female/aug_cgan/multi_B_A.png}
  \subfloat[AugCGAN Female-to-Male]{\includegraphics[width=.24\textwidth]{FIG/male2female/aug_cgan/multi_B_A.png}}
  \hfill
  \subfloat[CIN in low-level features]{\includegraphics[width=.24\textwidth]{FIG/male2female/lowlevel_cin_augcgan/lowlevel_cin_multi_A_B.png}}
  \hfill
  \subfloat[StochCGAN]{\includegraphics[width=.24\textwidth]{FIG/male2female/stoch_cgan/multi_A_B.png}}
  \caption{Generated female faces given a male face and multiple $z_b \sim p(z_b)$. (a) AugCGAN Male to many Females. (b) AugCGAN Female to many Males. (c) AugCGAN with CIN in low-level features. (d) StochCGAN with CIN.}
  \label{fig:m2f_comparison}
  \end{minipage}
\end{figure*}



% \begin{figure}

%   \begin{minipage}[b]{0.23\textwidth}
 
%   \subfloat[AugCGAN]{\includegraphics[width=.99\textwidth]{FIG/male2female/aug_cgan/multi_A_B.png}}
%   \end{minipage}
% %   \includegraphics[width=0.47\textwidth]{FIG/male2female/aug_cgan/multi_B_A.png}
%  \begin{minipage}[b]{0.23\textwidth}
%   \subfloat[StochCGAN]{\includegraphics[width=.99\textwidth]{FIG/male2female/stoch_cgan/multi_A_B.png}}
%   \end{minipage}
%   \caption{Comparision between(a) AugCGAN with CIN  (b) StochCGAN with CIN.}
%   \label{fig:m2f_comparison}
 
% \end{figure}




We study another image translation task of translating between male and female faces. Data is based on CelebA dataset~\cite{liu2015faceattributes} where we split it into two separate domains using provided attributes. Several key features distinguish this task from other image-translation tasks:
\begin{inlinelist}
\item there is no predefined correspondence in real data of each domain,
\item the relationship is many-to-many between domains, as we can map a male to female face, and vice-versa, in many possible ways, and
\item capturing realistic variations in generated faces requires transformations that go beyond simple color and texture changes.
\end{inlinelist}
(Fig.~\ref{fig:m2f_128}) shows results of applying our model to this task on $128 \times 128$ resolution CelebA images. We can see that our model depicts meaningful variations in generated faces without compromising their realistic appearance. On the other hand, while generated faces from Stochastic CycleGAN baseline look realistic, variations are limited and stale as shown in  (Fig.~\ref{fig:m2f_comparison}). Augmented CycleGAN gives diverse generations irrespective of the way we condition the latent code. Both conditional instance norm and concatenation with spatial replication gives meaningful variations. The detailed experimental setup is provided in the appendix \ref{sec:m2f_exp_details}
\todo{Why does our model work here? I believe we need to do ablation experiments which show which part of our model is most important here.}

% We used CelebA dataset\cite{liu2015faceattributes} to investigate the attribute transfer task. In this particular task only the gender feature varies across the domains. Unlike the case of edges-to-shoes here the relationship is many-to-many, one could generate multiple male faces from a female face with respect to other features and vice-versa. We successfully apply Augmented-CycleGAN to model these many-to-many relationships between both the domains. Figure ~\ref{fig:m2f_augcgan} depicts the meaningful variations captured by Augmented-CycleGAN from male to female conversion task and vice-versa without compromising on realistic generations.  Figure ~\ref{fig:m2f_stochcgan} shows the result of same task handled by stochastic-CycleGAN. Though the model produces realistic mappings, the variations are limited and stale unlike Augmented-CycleGAN[TODO: reason]. Detailed architecture and implementation details for this task are described in the appendix.





% \begin{figure}
% \centering
%   \begin{minipage}[b]{.45\textwidth}
%   \subfloat[Aug. CycleGAN]{\label{fig:m2f_augcgan_multi_male}\includegraphics[width=0.9\textwidth]{FIG/male2female/aug_cgan/multi_B_A.png}}
%   \end{minipage}
% \caption{Female to Male samples where $z_a \sim \pz(z_a)$.}
% \end{figure}

% \begin{figure}
% \centering
%   \begin{minipage}[b]{.45\textwidth}
%   \subfloat[Stoch. CycleGAN]{\label{fig:m2f_stochcgan_multi_female}\includegraphics[width=0.9\textwidth]{FIG/male2female/stoch_cgan/multi_A_B.png}}
%   \end{minipage}
% \caption{Male to Female samples where $z_a \sim \pz(z_a)$.}
% \end{figure}

% \begin{figure}
% \centering
%   \begin{minipage}[b]{.45\textwidth}
%   \subfloat[Stoch. CycleGAN]{\label{fig:m2f_stochcgan_multi_male}\includegraphics[width=0.9\textwidth]{FIG/male2female/stoch_cgan/multi_B_A.png}}
%   \end{minipage}
% \caption{Female to Male samples where $z_a \sim \pz(z_a)$.}
% \end{figure}

% \begin{figure}
% \centering
%   \begin{minipage}[b]{.2\textwidth}
%   \subfloat[Male to Female]{\label{fig:e2s_augcgan_cycle}\includegraphics[width=0.9\textwidth]{FIG/male2female/cycle_fem.png}}
%   \end{minipage}
% \begin{minipage}[b]{.2\textwidth}
%   \subfloat[Female to Male]{\label{fig:e2s_stochcgan_cycle}\includegraphics[width=0.9\textwidth]{FIG/male2female/cycle_male.png}}
%   \end{minipage}
% \caption{Forward and Backward Cycles. }
% \end{figure}



\subsection{Attributes-to-Faces}
\todo{describe experiment setting}

\begin{table}[h]
\centering
\begin{tabular}{lcc}
    \toprule
    \textbf{Model} & \multicolumn{2}{c}{\textbf{P@10}} \\
    		       &   $s =$ 1\% & $s = $ 10\% \\
    \midrule
    Triple-GAN$^\dagger$    & 40.97 & 62.13 \\
    $\Delta$-GAN$^\dagger$  & 53.21 & 63.68 \\
    \midrule
    Baseline Classifier  & 63.36 & 67.34 \\
	AugCGAN              & \textbf{64.28} & \textbf{68.83} \\
    \bottomrule
  \end{tabular}
  \caption{Semi-supervised attribute prediction on CelebA with supervision $s=$ 1\% and 10\% . $^\dagger$From \citep{gan2017triangle}.}
  \label{tab:shoe_recons}
\end{table}

\todo{Add generated faces from attributes.}

\todo{Add reconstructed faces (in appendix probably)}

==> amjad-approach.tex <==
Our proposed model has four components: two mappings $\Fz: \A \times \Zb \mapsto \B$ and $\Gz: \B \times \Za \mapsto \A$, which are the conditional generators of items in each domain. These models are similar to those used in Stochastic CycleGAN. We also have two encoders $\Ea:\A \times \B \mapsto \Za$ and $\Eb:\A \times \B \mapsto \Zb$, that will be used to correctly optimize cycle-consistency.
All components are parameterized with neural networks and illustrated in Fig.~\ref{fig:augmented_cycle_gan}.
We define mappings over augmented spaces in our model as follows. Let $\pz(z_a)$ and $\pz(z_b)$ be standard Gaussian priors over items of $\Za$ and $\Zb$, which are marginally independent from $\pdata(b)$ and $\pdata(a)$, respectively. Given a pair $(a, z_b) \sim \pdata(a)\pz(z_b)$, 
%\footnote{We assume marginal independence between $\pdata(a)$ and $\pz(z_b)$, and $\pdata(b)$ and $\pz(z_a)$.} 
we generate a pair $(\tilde{b}, \tilde{z}_a)$ by: 
\begin{align}
\tilde{b} &= \Fz(a, z_b),\; \tilde{z}_a = \Ea(a, \tilde{b}).
\label{eq:aug_cgan_forward}
\end{align}
That is, we first generate a sample in domain $\B$, then we use it along with $a$ to infer latent code $\tilde{z}_a$. Note here that by sampling different $z_b \sim \pz(z_b)$, we can generate multiple $\tilde{b}$'s conditioned on the same $a$. In addition, given the pair $(a, \tilde{b})$, we can recover information about $a$ which is not captured in $\tilde{b}$. This is important for reconstructing $a$ as we will see in Sec~\ref{sec:aug_cgan_cycle}.
Similarly, given a pair $(b, z_a)\sim \pdata(b)\pz(z_a)$, we generate a pair $(\tilde{a}, \tilde{z}_b)$ by: 
\begin{align}
\tilde{a} &= \Gz(b, z_a),\; \tilde{z}_b = \Eb(b, \tilde{a}).
\end{align}
Learning in Augmented CycleGAN follows a similar approach to CycleGAN of optimizing both marginal matching and cycle-consistency losses, albeit over augmented spaces. We describe in the following these objectives in detail.

\subsubsection{Marginal Matching Loss}
Marginal matching over augmented space $\B \times \Za$ ensures that the distribution of generated pairs $(\tilde{b}, \tilde{z}_a)$ matches the priors $(b,z_a) \sim \pdata(b)\pz(z_a)$.
We also adopt an adversarial approach for marginal matching over $\B \times \Za$ where we use two independent discriminators $D_\B$ and $D_{\Za}$ to match generated pairs to real samples from the marginally independent priors $\pdata(b)$ and $\pz(z_a)$, respectively. Marginal matching loss over $\B$ is given by: 
\begin{align}
\label{eq:aug_cgan_gan_b}
  \loss_{\text{GAN}}^B(\Fz, D_\B) = \E_{b \sim \pdata(b)} &\Big[ \log D_\B(b) \Big] +\nonumber \\
  \E_{ \substack{a \sim \pdata(a) \\ z_b \sim p(z_b)}} &\Big[ \log(1- D_\B(\Fz(a,z_b))) \Big].
\end{align}
Marginal matching over $\Za$ is given by:
\begin{align}
\label{eq:aug_cgan_gan_z}
  \loss_{\text{GAN}}^{\Za}(\Ea, \Fz, D_{\Za}) = &\E_{z_a \sim \pz(z_a)} \Big[ \log D_{\Za} \Big] + \nonumber \\ 
  &\E_{ \substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \Big[ \log(1- D_{\Za}(\tilde{z}_a)) \Big], %\nonumber \\
  %\tilde{z}_a =& \Ea(a, \tilde{b}), \nonumber \\
  %\tilde{b} =& \Gz(a, z_b).
\end{align}
where $\tilde{z}_a$ is defined by Eqn~\ref{eq:aug_cgan_forward}.
As in CycleGAN, the goal of marginal matching over $\B$ is to insure that generated samples $\tilde{b}$ are realistic. 
For latent codes $\tilde{z}_a$, however, marginal matching acts as a regularization term over the encoder, which ensures that encoding distribution matches a simple prior $\pz(z_a)$. This is similar to adversarial regularization of latent codes in adversarial autoencoders~\citep{makhzani2015adversarial}.
Similarly, we define losses $\loss_{\text{GAN}}^A(\Gz, D_\A)$ and $\loss_{\text{GAN}}^{\Zb}(\Eb, \Gz, D_{\Zb})$ for marginal matching over $\A \times \Zb$.

\subsubsection{Cycle-Consistency Loss} \label{sec:aug_cgan_cycle}
%The main motivation for performing cycle-consistency on augmented spaces is make sure that both source domain and latent space are used in generating samples.
We define two cycle-consistency constraints in Augmented CycleGAN starting from each of the two augmented spaces as shown in Fig.~\ref{fig:augmented_cycle_gan}. 
In cycle-consistency starting from $\A \times \Zb$, we ensure that given a pair $(a,z_b) \sim \pdata(a)\pz(z_b)$, the model is able to produce a faithful reconstruction of it after being mapped to $(\tilde{b}, \tilde{z_a})$. For cycle-consistency starting from $\A \times \Zb$, we define the following two losses. The first for reconstructing $a \sim \pdata(a)$:
\begin{align}
\label{eq:aug_cgan_fwd_cycle}
&\loss_{\text{CYC}}^A(\Fz, \Gz, \Ea) = \E_{\substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \Big[ \big\| a' - a \big\|_1  \Big], \nonumber \\ %\; \text{where:} \nonumber \\
%\intertext{where:}
\tilde{b} &= \Fz(a, z_b), \;\tilde{z}_a = \Ea(a, \tilde{b}),\; a' = \Gz(\tilde{b}, \tilde{z}_a).
% a' &= \Gz(\tilde{b}, \tilde{z}_a), \nonumber \\
% \tilde{b} &= \Fz(a, z_b), \nonumber \\
% \tilde{z}_a &= \Ea(a, \tilde{b}).
\end{align}
The second loss is for reconstructing $z_b \sim \pz(z_b)$:
\begin{align}
\label{eq:aug_cgan_fwd_cycle_z}
\loss_{\text{CYC}}^{\Zb}(\Fz, \Eb) =& \E_{\substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \Big[ \big\| z_b' - z_b \big\|_1  \Big], \nonumber \\ %\; \text{where:} \nonumber \\
%\intertext{where:}
z_b' = \Eb(a, \tilde{b}),& \;\;\; \tilde{b} = \Fz(a, z_b).
\end{align}
Just like in CycleGAN, the cycle loss in Eqn.~\ref{eq:aug_cgan_fwd_cycle} enforces the dependency of generated samples in $\B$ on samples of $\A$. Thanks to the encoder $\Ea$, the model is able to reconstruct $a$ because it can recover information loss in generated $\tilde{b}$ through $\tilde{z}_a$.
%In this sense, Augmented CycleGAN reduces the information bottleneck which domain $\B$ imposes in CycleGAN and Stochastic CycleGAN. 
On the other hand, the cycle loss in Eqn.~\ref{eq:aug_cgan_fwd_cycle_z} 
enforces the dependency of a generated sample $\tilde{b}$ on the given latent code $z_b$. Essentially, it increases the mutual information between $z_b$ and $b$ conditioned on $a$, i.e. $I(b,z_b|a)$~\citep{chen2016infogan,li2017alice}.
% Likewise, we define backward cycle-consistency in Augmented CycleGAN with the following two losses:
% \begin{align}
% \label{eq:aug_cgan_bwd_cycle}
% \loss_{\overleftarrow{\text{Cycle}}}(\Fz, \Gz, \Eb) &= \E_{\substack{b \sim \pdata(b)\\ z_a \sim \pz(z_a)}} \Big[ \big\| b' - b \big\|_1  \Big], \nonumber \\ %\; \text{where:} \nonumber \\
% %\intertext{where:}
% b' &= \Fz(\tilde{a}, \tilde{z}_b), \nonumber \\
% \tilde{a} &= \Gz(b, z_a), \nonumber \\
% \tilde{z}_b &= \Eb(\tilde{a}, b).
% \end{align}
% \begin{align}
% \label{eq:aug_cgan_bwd_cycle_z}
% \loss_{\overleftarrow{\text{z-cycle}}}(\Gz, \Ea) &= \E_{\substack{b \sim \pdata(b)\\ z_a \sim \pz(z_a)}} \Big[ \big\| z_a' - z_a \big\|_1  \Big], \nonumber \\ %\; \text{where:} \nonumber \\
% %\intertext{where:}
% z_a' &= \Ea(\tilde{a}, b), \nonumber \\
% \tilde{a} &= \Gz(b, z_a).
% \end{align}

% \subsubsection{Full Training Loss}
For training Augmented CycleGAN in the direction going from $\A \times \Zb$ to $\B \times \Za$, we optimize the loss:
%\begin{equation}
%\begin{aligned}
%\label{eq:aug_cgan_full_loss}
%&\min_{\substack{ \Fz, \Ea\\ \Gz, \Eb}}
%\max_{D_\B, D_{\Za}}
%\loss_{\text{GAN}}(\Fz, D_\B) +
%\loss_{\text{GAN}}(\Ea, \Fz, D_{\Za}) +\\
%& \gamma \loss_{\text{Cycle}^a}(\Fz, \Gz, \Ea) + \gamma_z\loss_{\text{Cycle}^{z_b}}(\Fz, \Eb) 
%\end{aligned}
%\end{equation}
\begin{equation}
\begin{split}
\label{eq:aug_cgan_full_loss}
&\loss_{\text{GAN}}^B(D_\B, \Fz) + \loss_{\text{GAN}}^{z_a}(D_{\Za}, \Ea, \Fz) \, + \\
& \gamma_1 \loss_{\text{CYC}}^A(\Fz, \Gz, \Ea) + \gamma_2 \loss_{\text{CYC}}^{z_b}(\Fz, \Eb),
\end{split}
\end{equation}
where $\gamma_1$ and $\gamma_2$ are a hyper-parameters used to balance objectives. We define a similar objective for the direction going from $\B \times \Za$ to $\A \times \Zb$, and train the model on both objectives simultaneously.

\begin{figure}[t!]
\centering
\includegraphics[width=0.45\textwidth]{FIG/ss_aug_cgan.pdf}
\caption{Augmented CycleGAN when pairs $(a, b) \sim p_d(a, b)$ from the true joint distribution are observed. % you can explain it if you want
}
\label{fig:ss_augmented_cycle_gan}
\end{figure}

\subsection{Semi-supervised Learning with Augmented CycleGAN}
Our model can be extended to the semi-supervised settings.
Given some paired data $(a, b) \sim \pdata(a,b)$ sampled from the true joint, we can define a supervision cost for the mapping $\Fz$ as follows:
\begin{align}
\label{eq:aug_cgan_fwd_sup}
\loss_{\text{SUP}}^A(\Fz, \Gz, \Ea) =& \E_{(a,b) \sim \pdata(a,b)} \Big[ \big\| a' - a \big\|_1  \Big], \nonumber \\ %\; \text{where:} \nonumber \\
%\intertext{where:}
\tilde{z}_a = \Ea(a, b),& \;\;\; a' = \Gz(b, \tilde{z}_a).
% a' &= \Gz(\tilde{b}, \tilde{z}_a), \nonumber \\
% \tilde{b} &= \Fz(a, z_b), \nonumber \\
% \tilde{z}_a &= \Ea(a, \tilde{b}).
\end{align}
We can also define a regularization cost for the encoder:
\begin{align}
\label{eq:aug_cgan_gan_z}
  \loss_{\text{GAN}}^{\Za}(\Ea, \Fz, D_{\Za}) = &\E_{z_a \sim \pz(z_a)} \Big[ \log D_{\Za} \Big] + \nonumber \\ 
  &\E_{ (a,b) \sim \pdata(a,b)} \Big[ \log(1- D_{\Za}(\tilde{z}_a)) \Big], \nonumber \\
  \tilde{z}_a =& \Ea(a, b). %\nonumber \\
  %\tilde{b} =& \Gz(a, z_b).
\end{align}
%where $\tilde{z}_a = \Ea(a,b)$

==> new-approach.tex <==


\subsection{Procedural Description}
Given a pair $(a, z_b) \sim p(a, z_b) = \pdata(a)p(z_b)$, we map to the augmented space $(B, Z_a)$,~i.e. producing a joint sample $(\tilde{b}, \tilde{z}_a)$ by the sequential application of $\F$ and $\Ea$:
\begin{align}
\tilde{b} &= \Fz(a, z_b),\; \tilde{z}_a = \Ea(a, \tilde{b}).
\label{eq:aug_cgan_forward}
\end{align}
That is, we first generate a sample $\tilde{b}$, then we use it along with $a$ to infer latent code $\tilde{z}_a$. The reason for the dependence of $z_a$ on both $a, \tilde{b}$ will be made more formal in Section~\ref{sec:aug_ae_perspective}, but intuitively, it is motivated by the fact that $z_a$ should contain information about $a$ that cannot be inferred from $\tilde{b}$.
% cycle consistency losses on the bottom reuse the previous but 
% wait, but the story stays the same just different presenation right? more brief than what I had, right?
% yes. i won't touch the story anymore
Marginal matching over augmented space $\B \times \Za$ ensures that the distribution of generated pairs $(\tilde{b}, \tilde{z}_a)$ matches the assumed prior $p(b, z_a) \sim \pdata(b)\pz(z_a)$.
We use two independent discriminators $D_\B$ and $D_{\Za}$ yielding:
\begin{equation}
\small
\begin{align}
\label{eq:aug_cgan_gan_b}
  \loss_{\text{GAN}}^B(\Fz, D_\B) = \E_{b \sim \pdata(b)} &\Big[ \log D_\B(b) \Big] +  \\
  \E_{ \substack{a \sim \pdata(a) \\ z_b \sim p(z_b)}} &\Big[ \log(1- D_\B(\Fz(a,z_b))) \Big].
\end{align}
\end{equation}
\begin{equation}
\small
\begin{align}
\small
\label{eq:aug_cgan_gan_z}
  \loss_{\text{GAN}}^{\Za}(\Ea, \Fz, D_{\Za}) = &\E_{z_a \sim \pz(z_a)} \Big[ \log D_{\Za}(z_a) \Big] + \\ 
  &\E_{ \substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \Big[ \log(1 - D_{\Za}(\tilde{z}_a)) \Big], %\nonumber \\
  %\tilde{z}_a =& \Ea(a, \tilde{b}), \nonumber \\
  %\tilde{b} =& \Gz(a, z_b).
\end{align}
\end{equation}

Cycle-consistency is defined by reconstructing the pair $(a, z_b)$. The reconstruction of $a$ uses the generated pair $(\tilde b, \tilde{z}_a)$. Formally:
\begin{equation}
\small
\label{eq:aug_cgan_fwd_cycle}
\loss_{\text{CYC}}^A(\Fz, \Gz, \Ea) = \E_{ \substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \big\| \G(\tilde{b}, \tilde{z}_a) - a \big\|_1,
\end{equation}
\begin{equation}
\small
\label{eq:aug_cgan_fwd_cycle_z}
\loss_{\text{CYC}}^{\Zb}(\Fz, \Eb) = \E_{\substack{a \sim \pdata(a)\\ z_b \sim \pz(z_b)}} \big\| \Eb(a, \tilde{b}) - z_b \big\|_1,
\end{equation}



==> other-approach.tex <==
In order to be able to optimize both marginal matching and cycle consistency when using stochastic mappings, we propose to augment domains $\A$ and $\B$ with latent spaces $\Zb$ and $\Za$ respectively and learn mappings between the augmented spaces $\A \times \Zb$ and $\B \times \Za$,~i.e. we learn to map between pairs of elements $(a, z_b) \in \A \times \Zb$ and $(b, z_a) \in \B \times \Za$. The auxiliary variable $z_b$ ($z_a$) contains features of domain $B$ that cannot be inferred from elements in $A$.

From a general standpoint, this approach can be described as learning mappings over \textit{augmented spaces} $\A \times \Zb$ and $\B \times \Za$ (Fig.~\ref{fig:augmented_cycle_gan}); hence, we call it \textit{Augmented CycleGAN}.

In the following, we first give a formal description procedural description of the model. Then we give a procedural description for the cycle starting from the augmented space $(A, Z_b)$. We leave to the reader the analogous derivation for the cycle starting from $(B, Z_a)$. Then, we will interpret our model in the context of adversarial autoencoders.

\subsection{Formal Description}
We assume there is an augmented underlying joint distribution $p(a, b, z_a, z_b)$ involving variables from the observed samples $A, B$ as well as auxiliary random variables $z_a, z_b$ taking values respectively in $\Za$ and $\Zb$. In our framework, we observe joint samples from \emph{augmented} spaces $(a, z_b) \sim p(a, z_b)$ and $(b, z_a) \sim p(b, z_a)$. We assume that these marginals factorize conveniently $p(a, z_b) = p_d(a)p(z_b)$, $p(b, z_a) = p_d(b)p(z_a)$. In order to uncover many-to-many mappings between $A$ and $B$, we propose to cycle over the augmented spaces $\A \times \Zb$ and $\B \times \Za$ in order to estimate the following conditionals: $\hat p(a, z_b | b, z_a)$, $\hat p(b, z_a | a, z_b)$. We assume these conditionals factorize as: $\hat p(a, z_b | b, z_a) =  p(z_b | b, a) p(a | b, z_a)$.

